Visual Point Cloud Forecasting enables Scalable Autonomous Driving

In contrast to extensive studies on general vision, pre-training for scalable visual autonomous driving remains seldom explored. Visual autonomous driving applications require features encompassing semantics, 3D geometry, and temporal information simultaneously for joint perception, prediction, and planning, posing dramatic challenges for pre-training. To resolve this, we bring up a new pre-training task termed as visual point cloud forecasting - predicting future point clouds from historical visual input. The key merit of this task captures the synergic learning of semantics, 3D structures, and temporal dynamics. Hence it shows superiority in various downstream tasks. To cope with this new problem, we present ViDAR, a general model to pre-train downstream visual encoders. It first extracts historical embeddings by the encoder. These representations are then transformed to 3D geometric space via a novel Latent Rendering operator for future point cloud prediction. Experiments show significant gain in downstream tasks, e.g., 3.1% NDS on 3D detection, ~10% error reduction on motion forecasting, and ~15% less collision rate on planning.

==> figures/framework.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{example-image-a}
  \caption{\textbf{Model architecture.} xx.
  }
  \label{fig:framework}
\end{figure*}

==> figures/latentrender_viz.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/files/LatentRendering_viz.pdf}
  % \vspace{-0.1in}
  \caption{\textbf{Effectiveness of \render.} Each triplet includes: \textbf{(left)} ray-shaped features raised during pre-training without using \render; \textbf{(middle)} 3D geometric-aware latent space produced by \render; \textbf{(right)} the corresponding point cloud. As illustrated, \render effectively constructs 3D scenes in latent space and correctly reflects 3D structures by feature responses.
  }
  \label{fig:latent_viz}
  % \vspace{-0.1in}
\end{figure*}

==> figures/teaser.tex <==
\begin{strip}
  \vspace{-15pt}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/files/teaser.pdf}\\
  \vspace{-5pt}
  \captionof{figure}{
  Forto learns to predict future point clouds from historical visual sequences using scales of obtainable Image-LiDAR pairs. With our \textit{LatentRender} design, this effectively extracts features capable of estimating motion, flow, and 3D geometry from visual inputs and in turn benefits downstream applications.
  
  Forto learns estimating motion, flow, and 3D geometry by predicting future point clouds from historical visual sequence inputs. By learning from scalable Image-LiDAR pairs, Forto shows superior performance on point cloud forecasting and downstream applications.
  
  takes a visual sequence as inputs and predicts future point clouds by estimating motion, flow, and 3D geometry, which in turn benefits downstream applications. \textbf{(Upper \& lower:)} Forto accurately estimates the relative motion between ego-vehicle and other moving vehicles (moving closer or keeping distance); \textbf{(Middle:)} Forto correctly predicts the future motion of ego-vehicle (turn right).
  }
  \vspace{-5pt}
  \label{fig:teaser}
\end{strip}

==> figures/vis.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=.5\linewidth]{example-image-a}
  % \vspace{-0.1in}
  \caption{Qualitative results.
  }
  \label{fig:vis}
  % \vspace{-0.1in}
\end{figure*}
